Fragmentation and Evolution of Molecular Clouds. II: The Effect of Dust Heating

We investigate the effect of heating by luminosity sources in a simulation of clustered star formation. Our heating method involves a simplified continuum radiative transfer method that calculates the dust temperature. The gas temperature is set by the dust temperature. We present the results of four simulations, two simulations assume an isothermal equation of state and the two other simulations include dust heating. We investigate two mass regimes, i.e., 84 Msun and 671 Msun, using these two different energetics algorithms. The mass functions for the isothermal simulations and simulations which include dust heating are drastically different. In the isothermal simulation, we do not form any objects with masses above 1 Msun. However, the simulation with dust heating, while missing some of the low-mass objects, forms high-mass objects (~20 Msun) which have a distribution similar to the Salpeter IMF. The envelope density profiles around the stars formed in our simulation match observed values around isolated, low-mass star-forming cores. We find the accretion rates to be highly variable and, on average, increasing with final stellar mass. By including radiative feedback from stars in a cluster-scale simulation, we have determined that it is a very important effect which drastically affects the mass function and yields important insights into the formation of massive stars.

==> figs-dust.tex <==
\clearpage




\clearpage
\clearpage


